Pre main sequence: Accretion & Outflows

Low-mass pre-main sequence (PMS) stars are strong X-ray sources, because they possess hot corona like their older main-sequence counterparts. Unique to young stars, however, are X-rays from accretion and outflows, and both processes are of pivotal importance for star and planet formation. We describe how X-ray data provide important insight into the physics of accretion and outflows. First, mass accreted from a circumstellar disk onto the stellar surface reaches velocities up to a few hundred km/s, fast enough to generate soft X-rays in the post-shock region of the accretion shock. X-ray observations together with laboratory experiments and numerical simulations show that the accretion geometry is complex in young stars. Specifically, the center of the accretion column is likely surrounded by material shielding the inner flow from view but itself also hot enough to emit X-rays. Second, X-rays are observed in two locations of protostellar jets: an inner stationary emission component probably related to outflow collimation and outer components, which evolve withing years and are likely related to working surfaces where the shock travels through the jet. Jet-powered X-rays appear to trace the fastest jet component and provide novel information on jet launching in young stars. We conclude that X-ray data will continue to be highly important for understanding star and planet formation, because they directly probe the origin of many emission features studied in other wavelength regimes. In addition, future X-ray missions will improve sensitivity and spectral resolution to probe key model parameters (e.g. velocities) in large samples of PMS stars.

==> Xrayhandbook/symbols.tex <==
\usepackage{xspace}

\newcommand{\sun}{$_{\odot}$\xspace}

\DeclareRobustCommand{\ion}[2]{%
\relax\ifmmode
\ifx\testbx\f@series
{\mathbf{#1\,\mathsc{#2}}}\else
{\mathrm{#1\,\mathsc{#2}}}\fi
\else\textup{#1\,{\mdseries\textsc{#2}}}%
\fi}

\def\degr{\hbox{$^\circ$}}
\def\arcmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\utw{\smash{\rlap{\lower5pt\hbox{$\sim$}}}}
\def\udtw{\smash{\rlap{\lower6pt\hbox{$\approx$}}}}
\def\fd{\hbox{$.\!\!^{\rm d}$}}
\def\fh{\hbox{$.\!\!^{\rm h}$}}
\def\fm{\hbox{$.\!\!^{\rm m}$}}
\def\fs{\hbox{$.\!\!^{\rm s}$}}
\def\fdg{\hbox{$.\!\!^\circ$}}
\def\farcm{\hbox{$.\mkern-4mu^\prime$}}
\def\farcs{\hbox{$.\!\!^{\prime\prime}$}}


\def\aj{AJ}%

          % Astronomical Journal

\def\araa{ARA\&A}%

          % Annual Review of Astron and Astrophys

\def\apj{ApJ}%

          % Astrophysical Journal

\def\apjl{ApJ}%

          % Astrophysical Journal, Letters

\def\apjs{ApJS}%

          % Astrophysical Journal, Supplement

\def\ao{Appl.~Opt.}%

          % Applied Optics

\def\apss{Ap\&SS}%

          % Astrophysics and Space Science

\def\aap{A\&A}%

          % Astronomy and Astrophysics

\def\aapr{A\&A~Rev.}%

          % Astronomy and Astrophysics Reviews

\def\aaps{A\&AS}%

          % Astronomy and Astrophysics, Supplement

\def\azh{AZh}%

          % Astronomicheskii Zhurnal

\def\baas{BAAS}%

          % Bulletin of the AAS

\def\jrasc{JRASC}%

          % Journal of the RAS of Canada

\def\memras{MmRAS}%

          % Memoirs of the RAS

\def\mnras{MNRAS}%

          % Monthly Notices of the RAS

\def\pra{Phys.~Rev.~A}%

          % Physical Review A: General Physics

\def\prb{Phys.~Rev.~B}%

          % Physical Review B: Solid State

\def\prc{Phys.~Rev.~C}%

          % Physical Review C

\def\prd{Phys.~Rev.~D}%

          % Physical Review D

\def\pre{Phys.~Rev.~E}%

          % Physical Review E

\def\prl{Phys.~Rev.~Lett.}%

          % Physical Review Letters

\def\pasp{PASP}%

          % Publications of the ASP

\def\pasj{PASJ}%

          % Publications of the ASJ

\def\qjras{QJRAS}%

          % Quarterly Journal of the RAS

\def\skytel{S\&T}%

          % Sky and Telescope

\def\solphys{Sol.~Phys.}%

          % Solar Physics

\def\sovast{Soviet~Ast.}%

          % Soviet Astronomy

\def\ssr{Space~Sci.~Rev.}%

          % Space Science Reviews

\def\zap{ZAp}%

          % Zeitschrift fuer Astrophysik

\def\nat{Nature}%

          % Nature

\def\iaucirc{IAU~Circ.}%

          % IAU Cirulars

\def\aplett{Astrophys.~Lett.}%

          % Astrophysics Letters

\def\apspr{Astrophys.~Space~Phys.~Res.}%

          % Astrophysics Space Physics Research

\def\bain{Bull.~Astron.~Inst.~Netherlands}%

          % Bulletin Astronomical Institute of the Netherlands

\def\fcp{Fund.~Cosmic~Phys.}%

          % Fundamental Cosmic Physics

\def\gca{Geochim.~Cosmochim.~Acta}%

          % Geochimica Cosmochimica Acta

\def\grl{Geophys.~Res.~Lett.}%

          % Geophysics Research Letters

\def\jcp{J.~Chem.~Phys.}%

          % Journal of Chemical Physics

\def\jgr{J.~Geophys.~Res.}%

          % Journal of Geophysics Research

\def\jqsrt{J.~Quant.~Spec.~Radiat.~Transf.}%

          % Journal of Quantitiative Spectroscopy and Radiative Trasfer

\def\memsai{Mem.~Soc.~Astron.~Italiana}%

          % Mem. Societa Astronomica Italiana

\def\nphysa{Nucl.~Phys.~A}%

          % Nuclear Physics A

\def\physrep{Phys.~Rep.}%

          % Physics Reports

\def\physscr{Phys.~Scr}%

          % Physica Scripta

\def\planss{Planet.~Space~Sci.}%

          % Planetary Space Science

\def\procspie{Proc.~SPIE}%

          % Proceedings of the SPIE

\let\astap=\aap

\let\apjlett=\apjl

\let\apjsupp=\apjs

\let\applopt=\ao

%

\uchyph=0

